Vision in the Era of Agents: Toward Recursive Self-Improvement

Large language model (LLM) agents have emerged as a paradigm for goal-directed problem solving, leveraging reasoning, planning, and tool use to accomplish complex tasks. Beyond text-based applications, these capabilities are increasingly being extended to visual domains, where visual agents ground their decisions and actions in images, videos, and interactive feedback. This paper provides a systematic overview of recent advances in these visual agents. We first conceptualize visual agents as systems in which one or more models operate within an associated agent harness. We then categorize mechanisms for improving agent capabilities by the depth of experience-driven change in these systems, distinguishing within-task adaptation, self-evolution, and recursive self-improvement (RSI). For each level, we review representative methods across visual understanding, generation, computer use, and embodied interaction, examining their sources of experience, targets of change, and underlying mechanisms. Relevant benchmarks and evaluation protocols are also summarized, providing a reference for evaluating visual agents across diverse tasks and settings. To support further research, resources are available at http://visual-agent-survey.github.io

==> links.tex <==
% Load in the manuscript preamble, after xcolor and before \begin{document}.
% Define clickable paper, code, and dataset icons without PDF link outlines.
\RequirePackage{fontawesome5}
\makeatletter
\@ifpackageloaded{hyperref}{}{\RequirePackage{hyperref}}
\makeatother
% Red internal references, green citations, and magenta URL text; no link outlines.
% Also apply when hyperref was loaded earlier by the main document.
\hypersetup{
  colorlinks=true,
  linkcolor=red,       % 章节、图表等交叉引用：红色
  citecolor=green,     % 论文引用 [33] 等：亮绿色
  urlcolor=magenta,
  filecolor=black,
  pdfborder={0 0 0},
  pdfborderstyle={/W 0}
}
% Scheme B: shared semantic colors for every resource icon and legend.
\definecolor{SurveyLinkPaper}{HTML}{3C6EAF}
\definecolor{SurveyLinkCode}{HTML}{3B7D6D}
\definecolor{SurveyLinkData}{HTML}{9272B1}
\newcommand{\SurveyPaperIcon}{\textcolor{SurveyLinkPaper}{\faIcon{file-alt}}}
\newcommand{\SurveyCodeIcon}{\textcolor{SurveyLinkCode}{\faIcon{github}}}
\newcommand{\SurveyDataIcon}{\textcolor{SurveyLinkData}{\faIcon{database}}}
\providecommand{\benchpaper}[1]{\href{#1}{\raisebox{0.05ex}{\scriptsize\SurveyPaperIcon}}}
\providecommand{\benchcode}[1]{\href{#1}{\raisebox{0.05ex}{\scriptsize\SurveyCodeIcon}}}

\providecommand{\benchdata}[1]{\href{#1}{\raisebox{0.05ex}{\scriptsize\SurveyDataIcon}}}

% Shared fixed-width Paper / Code / Data slots; unavailable links remain black dashes.
\newcommand{\TableLinkSlot}[2]{%
  \makebox[1.1em][c]{%
    \if\relax\detokenize{#1}\relax
      \textcolor{black}{\textnormal{-}}%
    \else
      \href{#1}{\raisebox{0.03ex}{\scriptsize #2}}%
    \fi}}
\newcommand{\SurveyTableLinks}[4][]{%
  \mbox{\TableLinkSlot{#2}{\SurveyPaperIcon}\hspace{0.12em}%
  \TableLinkSlot{#3}{\SurveyCodeIcon}\hspace{0.12em}%
  \TableLinkSlot{#4}{\SurveyDataIcon}%
  \if\relax\detokenize{#1}\relax\else
    \rlap{\textcolor{black}{\textsuperscript{#1}}}\fi}}
\newcommand{\TableLinksLegend}{%
  \textit{Links:} \SurveyPaperIcon\,Paper\quad
  \SurveyCodeIcon\,Code\quad
  \textcolor{black}{-}\,Not identified in reviewed sources.}
\newcommand{\TableLinksWithDataLegend}{%
  \textit{Links:} \SurveyPaperIcon\,Paper\quad
  \SurveyCodeIcon\,Code\quad
  \SurveyDataIcon\,Data\quad
  \textcolor{black}{-}\,Not identified.}
\newcommand{\TableDatasetLinksLegend}{%
  \textit{Links:} \SurveyPaperIcon\,Paper\quad
  \SurveyCodeIcon\,Code\quad
  \SurveyDataIcon\,Data\quad
  \textcolor{black}{-}\,Unavailable.}
\newcommand{\TablePaperCodeLinks}[2]{%
  \mbox{\TableLinkSlot{#1}{\SurveyPaperIcon}\hspace{0.12em}%
  \TableLinkSlot{#2}{\SurveyCodeIcon}}}
\newcommand{\DeclareTableWorkLinks}[4]{%
  \expandafter\gdef\csname TableWorkLinks@#1\endcsname{\TablePaperCodeLinks{#2}{#3}}%
  \expandafter\gdef\csname TableWorkLinksWithData@#1\endcsname{\SurveyTableLinks{#2}{#3}{#4}}}
\newcommand{\TableWorkLinks}[1]{%
  \ifcsname TableWorkLinks@#1\endcsname
    \csname TableWorkLinks@#1\endcsname
  \else
    \TablePaperCodeLinks{}{}%
  \fi}
\newcommand{\TableWorkLinksWithData}[1]{%
  \ifcsname TableWorkLinksWithData@#1\endcsname
    \csname TableWorkLinksWithData@#1\endcsname
  \else
    \SurveyTableLinks{}{}{}%
  \fi}
% Shared resource declarations; maintained together with the macros in links.tex.
% Verified resource URLs shared by bibliography key.
% Work tables can display Paper / Code, or opt into Paper / Code / Data.
% The dataset table retains its explicit Paper / Code / Data URLs.
\DeclareTableWorkLinks{AAAI2026Agentsama}{https://ojs.aaai.org/index.php/AAAI/article/view/40187}{https://github.com/pockyitachi/Agent-SAMA}{}
\DeclareTableWorkLinks{AAAI2026CoEPG}{https://arxiv.org/abs/2511.10705}{}{}
\DeclareTableWorkLinks{AAAI2026Dgara}{https://arxiv.org/abs/2511.16590v1}{https://github.com/sen0609/D-GARA}{https://github.com/sen0609/D-GARA/blob/main/D-GARA-152.json}
\DeclareTableWorkLinks{AAAI2026Genmac}{https://arxiv.org/abs/2412.04440}{https://github.com/Karine-Huang/GenMAC}{}
\DeclareTableWorkLinks{AAAI2026LookAsYouThink}{https://arxiv.org/abs/2511.12003}{https://github.com/PolarisLiu1/LAT}{}
\DeclareTableWorkLinks{AAAI2026Mobileagentrag}{https://arxiv.org/abs/2511.12254}{https://github.com/george13zyx/MAR}{}
\DeclareTableWorkLinks{AAAI2026PerTouch}{https://arxiv.org/abs/2511.12998}{https://github.com/Auroral703/PerTouch}{}
\DeclareTableWorkLinks{ACL2024VisualWebArena}{https://aclanthology.org/2024.acl-long.50/}{https://github.com/web-arena-x/visualwebarena}{https://github.com/web-arena-x/visualwebarena/tree/main/config_files}
\DeclareTableWorkLinks{ACL2026ConflictAware}{https://aclanthology.org/2026.acl-long.1306/}{https://github.com/makexine/CDRs}{}
\DeclareTableWorkLinks{ACL2026DocLens}{https://arxiv.org/abs/2511.11552}{}{}
\DeclareTableWorkLinks{ACL2026LongVideoAgent}{https://arxiv.org/abs/2512.20618}{https://github.com/longvideoagent/LongVideoAgent}{}
\DeclareTableWorkLinks{ACL2026ReLook}{https://aclanthology.org/2026.acl-long.1167/}{}{}
\DeclareTableWorkLinks{CVPR2025ComfyBench}{https://openaccess.thecvf.com/content/CVPR2025/html/Xue_ComfyBench_Benchmarking_LLM-based_Agents_in_ComfyUI_for_Autonomously_Designing_Collaborative_CVPR_2025_paper.html}{https://github.com/xxyQwQ/ComfyBench}{https://github.com/xxyQwQ/ComfyBench/tree/main/dataset}
\DeclareTableWorkLinks{CVPR2025Thinking}{https://arxiv.org/abs/2412.14171}{https://github.com/vision-x-nyu/thinking-in-space}{https://huggingface.co/datasets/nyu-visionx/VSI-Bench}
\DeclareTableWorkLinks{CVPR2025VideoMME}{https://openaccess.thecvf.com/content/CVPR2025/html/Fu_Video-MME_The_First-Ever_Comprehensive_Evaluation_Benchmark_of_Multi-modal_LLMs_in_CVPR_2025_paper.html}{https://github.com/MME-Benchmarks/Video-MME}{https://huggingface.co/datasets/lmms-eval/Video-MME}
\DeclareTableWorkLinks{CVPR2026AGENTSAFE}{https://openaccess.thecvf.com/content/CVPR2026/html/Ying_AGENTSAFE_Benchmarking_the_Safety_of_Embodied_Agents_on_Hazardous_Instructions_CVPR_2026_paper.html}{}{}
\DeclareTableWorkLinks{CVPR2026Dejavu}{https://arxiv.org/abs/2510.10181}{}{}
\DeclareTableWorkLinks{CVPR2026Explore}{https://arxiv.org/abs/2601.10744}{https://github.com/wangsen99/LMEE}{https://huggingface.co/datasets/wangsen99/LMEE-Bench}
\DeclareTableWorkLinks{CVPR2026FLARE}{https://arxiv.org/abs/2608.26645}{}{}
\DeclareTableWorkLinks{CVPR2026Jarvisevo}{https://arxiv.org/abs/2511.23002}{https://github.com/LYL1015/JarvisEvo}{https://huggingface.co/datasets/JarvisEvo/ArtEdit-Bench}
\DeclareTableWorkLinks{CVPR2026META}{https://openaccess.thecvf.com/content/CVPR2026/html/Huang_META_Meta_Evolution_of_Tool_Trajectory_Adaptation_for_Long-Video_Understanding_CVPR_2026_paper.html}{}{}
\DeclareTableWorkLinks{CVPR2026MMReCoder}{https://arxiv.org/abs/2604.01600}{https://github.com/ZitianTang/MMReCoder}{}
\DeclareTableWorkLinks{CVPR2026OSOracle}{https://arxiv.org/abs/2512.16295}{https://github.com/numbmelon/OS-Oracle}{https://huggingface.co/datasets/OS-Copilot/OS-Critic-Bench}
\DeclareTableWorkLinks{CVPR2026VISTA}{https://arxiv.org/abs/2510.15831}{}{}
\DeclareTableWorkLinks{CVPR2026ViLoMem}{https://arxiv.org/abs/2511.21678}{https://github.com/weihao-bo/ViLoMem}{}
\DeclareTableWorkLinks{CVPR2026Videoarm}{https://arxiv.org/abs/2512.12360}{https://github.com/MILVLG/videoarm}{}
\DeclareTableWorkLinks{CVPR2026WorldMM}{https://arxiv.org/abs/2512.02425}{https://github.com/wgcyeo/WorldMM}{}
\DeclareTableWorkLinks{CoLLAs2022CORA}{https://proceedings.mlr.press/v199/powers22b.html}{https://github.com/AGI-Labs/continual_rl}{}
\DeclareTableWorkLinks{ECCV2024BLINK}{https://arxiv.org/abs/2404.12390}{https://github.com/zeyofu/BLINK_Benchmark}{https://huggingface.co/datasets/BLINK-Benchmark/BLINK}
\DeclareTableWorkLinks{ECCV2026FindingDory}{https://arxiv.org/abs/2506.15635}{https://github.com/findingdory-benchmark/findingdory-habitat}{https://huggingface.co/datasets/yali30/findingdory}
\DeclareTableWorkLinks{ECCV2026Openearthagent}{https://arxiv.org/abs/2602.17665}{https://github.com/mbzuai-oryx/OpenEarthAgent}{}
\DeclareTableWorkLinks{ICCV2025VSP}{https://openaccess.thecvf.com/content/ICCV2025/html/Wu_VSP_Diagnosing_the_Dual_Challenges_of_Perception_and_Reasoning_in_ICCV_2025_paper.html}{https://github.com/UCSB-NLP-Chang/Visual-Spatial-Planning}{https://github.com/UCSB-NLP-Chang/Visual-Spatial-Planning/tree/main/VSP-main}
\DeclareTableWorkLinks{ICLR2025AndroidWorld}{https://arxiv.org/abs/2405.14573}{https://github.com/google-research/android_world}{https://github.com/google-research/android_world/tree/main/android_world/task_evals}
\DeclareTableWorkLinks{ICLR2025MMSearch}{https://proceedings.iclr.cc/paper_files/paper/2025/file/04e6525463afaa460b5a2e6868b18f18-Paper-Conference.pdf}{https://github.com/CaraJ7/MMSearch}{https://huggingface.co/datasets/CaraJ/MMSearch}
\DeclareTableWorkLinks{ICLR2025VisualAgentBench}{https://proceedings.iclr.cc/paper_files/paper/2025/hash/eea71dc576381b88f2a0ca4dedc2140d-Abstract-Conference.html}{https://github.com/THUDM/VisualAgentBench}{}
\DeclareTableWorkLinks{ICLR2026CoDA}{https://arxiv.org/abs/2510.03194}{}{}
\DeclareTableWorkLinks{ICLR2026ComputerRL}{https://arxiv.org/abs/2508.14040}{https://github.com/THUDM/ComputerRL}{}
\DeclareTableWorkLinks{ICLR2026Darwin}{https://arxiv.org/abs/2505.22954}{https://github.com/jennyzzt/dgm}{}
\DeclareTableWorkLinks{ICLR2026Error}{https://arxiv.org/abs/2509.01350}{}{}
\DeclareTableWorkLinks{ICLR2026Huxley}{https://arxiv.org/abs/2510.21614}{https://github.com/metauto-ai/HGM}{}
\DeclareTableWorkLinks{ICLR2026LongHorizonUI}{https://openreview.net/pdf?id=BK7Mk5d4WE}{https://github.com/kane2kang/LongHorizonUI}{}
\DeclareTableWorkLinks{ICLR2026Memoryvla}{https://arxiv.org/abs/2508.19236}{https://github.com/shihao1895/MemoryVLA}{}
\DeclareTableWorkLinks{ICLR2026OSWorldMCP}{https://arxiv.org/abs/2510.24563}{https://github.com/X-PLUG/OSWorld-MCP}{}
\DeclareTableWorkLinks{ICLR2026P2p}{https://arxiv.org/abs/2505.17104}{https://github.com/multimodal-art-projection/P2P}{}
\DeclareTableWorkLinks{ICLR2026Polyskill}{https://arxiv.org/abs/2510.15863}{https://github.com/simonucl/PolySkill}{}
\DeclareTableWorkLinks{ICLR2026Scenethesis}{https://arxiv.org/abs/2505.02836}{}{}
\DeclareTableWorkLinks{ICLR2026Seeing}{https://arxiv.org/abs/2508.09736}{https://github.com/ByteDance-Seed/m3-agent}{https://huggingface.co/datasets/ByteDance-Seed/M3-Bench}
\DeclareTableWorkLinks{ICLR2026VisualSelfRefine}{https://arxiv.org/abs/2602.16455}{https://github.com/InternLM/VSR}{}
\DeclareTableWorkLinks{ICLR2026Visualprompter}{https://arxiv.org/abs/2506.23138}{https://github.com/teheperinko541/VisualPrompter}{}
\DeclareTableWorkLinks{ICML2023VIMA}{https://proceedings.mlr.press/v202/jiang23b.html}{https://github.com/vimalabs/VIMABench}{https://huggingface.co/datasets/VIMA/VIMA-Data}
\DeclareTableWorkLinks{ICML2025Agent}{https://arxiv.org/abs/2409.07429}{https://github.com/zorazrw/agent-workflow-memory}{}
\DeclareTableWorkLinks{ICML2025EmbodiedBench}{https://arxiv.org/abs/2502.09560}{https://github.com/EmbodiedBench/EmbodiedBench}{https://huggingface.co/datasets/EmbodiedBench/EB-ALFRED}
\DeclareTableWorkLinks{ICML2025MedRAX}{https://arxiv.org/abs/2502.02673}{https://github.com/bowang-lab/MedRAX}{}
\DeclareTableWorkLinks{ICML2026Recovering}{https://arxiv.org/abs/2605.29447}{https://github.com/AlibabaResearch/RoTS}{}
\DeclareTableWorkLinks{NeurIPS2023LIBERO}{https://arxiv.org/abs/2306.03310}{https://github.com/Lifelong-Robot-Learning/LIBERO}{https://libero-project.github.io/datasets}
\DeclareTableWorkLinks{NeurIPS2023Mind2Web}{https://papers.neurips.cc/paper_files/paper/2023/hash/5950bf290a1570ea401bf98882128160-Abstract-Datasets_and_Benchmarks.html}{https://github.com/OSU-NLP-Group/Mind2Web}{https://huggingface.co/datasets/osunlp/Mind2Web}
\DeclareTableWorkLinks{NeurIPS2023Reflexion}{https://arxiv.org/abs/2303.11366}{https://github.com/noahshinn024/reflexion}{}
\DeclareTableWorkLinks{NeurIPS2024LongVideoBench}{https://proceedings.neurips.cc/paper_files/paper/2024/file/329ad516cf7a6ac306f29882e9c77558-Paper-Datasets_and_Benchmarks_Track.pdf}{https://github.com/longvideobench/LongVideoBench}{https://huggingface.co/datasets/longvideobench/LongVideoBench}
\DeclareTableWorkLinks{NeurIPS2024OSWorld}{https://arxiv.org/html/2404.07972v2}{https://github.com/xlang-ai/OSWorld}{https://github.com/xlang-ai/OSWorld/tree/main/evaluation_examples}
\DeclareTableWorkLinks{NeurIPS2024On}{https://proceedings.neurips.cc/paper_files/paper/2024/hash/a79f3ef3b445fd4659f44648f7ea8ffd-Abstract-Datasets_and_Benchmarks_Track.html}{https://github.com/google-research/google-research/tree/master/android_control}{https://console.cloud.google.com/storage/browser/gresearch/android_control}
\DeclareTableWorkLinks{NeurIPS2024Visual}{https://arxiv.org/abs/2406.09403}{https://github.com/Yushi-Hu/VisualSketchpad}{}
\DeclareTableWorkLinks{NeurIPS2025GUIActor}{https://arxiv.org/abs/2506.03143}{https://github.com/microsoft/GUI-Actor}{}
\DeclareTableWorkLinks{NeurIPS2025GUIReflection}{https://arxiv.org/html/2506.08012}{https://github.com/penghao-wu/GUI_Reflection}{https://huggingface.co/datasets/craigwu/GUI_Reflection_Task_Suite_Benchmark}
\DeclareTableWorkLinks{NeurIPS2025GUIRise}{https://arxiv.org/abs/2510.27210}{https://github.com/Leon022/GUI-Rise-code}{}
\DeclareTableWorkLinks{NeurIPS2025MedAgentBoard}{https://arxiv.org/html/2505.12371}{https://github.com/yhzhu99/MedAgentBoard}{https://zenodo.org/records/22299495}
\DeclareTableWorkLinks{NeurIPS2025StreamForest}{https://arxiv.org/abs/2509.24871}{https://github.com/MCG-NJU/StreamForest}{https://huggingface.co/datasets/MCG-NJU/StreamForest-Annodata}
\DeclareTableWorkLinks{NeurIPS2025VLMs}{https://arxiv.org/abs/2507.13361}{https://github.com/princeton-vl/vlmtunnel}{https://huggingface.co/datasets/princeton-vl/vlmtunnel}
\DeclareTableWorkLinks{NeurIPS2025VideoLucy}{https://arxiv.org/abs/2510.12422}{https://github.com/worldbench/VideoLucy}{https://huggingface.co/datasets/jlongzuo/EgoMem}
\DeclareTableWorkLinks{NeurIPS2026AUTOMEM}{https://arxiv.org/abs/2607.01224}{https://github.com/autoLearnMem/AutoMem}{}
\DeclareTableWorkLinks{NeurIPS2026AgentVista}{https://arxiv.org/abs/2602.23166}{https://github.com/hkust-nlp/AgentVista}{https://huggingface.co/datasets/Warrieryes/AgentVista}
\DeclareTableWorkLinks{NeurIPS2026EvoCUA}{https://arxiv.org/abs/2601.15876}{https://github.com/meituan/EvoCUA}{}
\DeclareTableWorkLinks{NeurIPS2026REINS}{https://neurips.cc/virtual/2026/poster/153736}{}{}
\DeclareTableWorkLinks{NeurIPS2026VLACorrector}{https://arxiv.org/abs/2607.01804}{https://github.com/ZJU-OmniAI/vla-corrector}{}
\DeclareTableWorkLinks{RAL2022CALVIN}{https://arxiv.org/abs/2112.03227}{https://github.com/mees/calvin}{https://github.com/mees/calvin/tree/main/dataset}
\DeclareTableWorkLinks{added_anwar2025remembr}{https://arxiv.org/abs/2409.13682}{https://github.com/NVIDIA-AI-IOT/remembr}{}
\DeclareTableWorkLinks{added_chhikara2025mem0}{https://arxiv.org/abs/2504.19413}{https://github.com/mem0ai/mem0}{}
\DeclareTableWorkLinks{added_guo2026vlaw}{https://arxiv.org/abs/2602.12063}{https://github.com/Robert-gyj/Ctrl-World}{}
\DeclareTableWorkLinks{added_guo2026webcogreasoner}{https://arxiv.org/abs/2508.01858}{https://github.com/Gnonymous/Web-CogReasoner}{}
\DeclareTableWorkLinks{added_ma2026vita}{https://arxiv.org/abs/2511.19859}{}{}
\DeclareTableWorkLinks{added_prabhu2026walt}{https://arxiv.org/abs/2510.01524}{https://github.com/SalesforceAIResearch/WALT}{}
\DeclareTableWorkLinks{added_qin2026tdatr}{https://arxiv.org/abs/2603.22819}{https://github.com/Chunchunwumu/TDATR}{}
\DeclareTableWorkLinks{added_rana2023sayplan}{https://proceedings.mlr.press/v229/rana23a.html}{}{}
\DeclareTableWorkLinks{added_shen2026agenticretoucher}{https://arxiv.org/abs/2601.02046}{https://github.com/MediaX-SJTU/Agentic-Retoucher}{}
\DeclareTableWorkLinks{added_shi2026duogen}{https://openaccess.thecvf.com/content/CVPR2026/papers/Shi_DuoGen_Towards_Autonomous_Interleaved_Multimodal_Generation_CVPR_2026_paper.pdf}{}{}
\DeclareTableWorkLinks{added_song2024moviechat}{https://arxiv.org/abs/2307.16449}{https://github.com/wenhaochai/MovieChat}{https://huggingface.co/datasets/Enxin/MovieChat-1K-test}
\DeclareTableWorkLinks{added_tang2026cccaption}{https://arxiv.org/abs/2602.21655}{https://github.com/ZhijiangTang/CCCaption}{}
\DeclareTableWorkLinks{added_wang2025jarvisone}{https://arxiv.org/abs/2311.05997}{https://github.com/CraftJarvis/JARVIS-1}{}
\DeclareTableWorkLinks{added_wang2026treevgr}{https://arxiv.org/abs/2507.07999}{https://github.com/Haochen-Wang409/TreeVGR}{}
\DeclareTableWorkLinks{added_zhang2026widget2code}{https://arxiv.org/abs/2512.19918}{https://github.com/Djanghao/widget2code}{}
\DeclareTableWorkLinks{awais2025foundation}{https://arxiv.org/abs/2307.13721}{https://github.com/awaisrauf/Awesome-CV-Foundational-Models}{}
\DeclareTableWorkLinks{bai2026deltareplay}{https://arxiv.org/abs/2610.11707}{https://arxiv.org/src/2610.11707v1/anc/code/README.md}{}
\DeclareTableWorkLinks{ding2026zetta}{https://arxiv.org/abs/2608.16590}{https://github.com/air-embodied-brain/Zetta-Embodiment}{}
\DeclareTableWorkLinks{dong2026revealing}{https://aclanthology.org/2026.acl-long.2087/}{https://github.com/dddraxxx/Awesome-Image-Grounded-CoT}{}
\DeclareTableWorkLinks{fan2026evolving}{https://arxiv.org/abs/2603.05860}{}{}
\DeclareTableWorkLinks{fu2026video}{https://arxiv.org/abs/2604.05015}{https://github.com/MME-Benchmarks/Video-MME-v2}{https://huggingface.co/datasets/MME-Benchmarks/Video-MME-v2}
\DeclareTableWorkLinks{gu2022vlnsurvey}{https://aclanthology.org/2022.acl-long.524/}{https://github.com/UCSB-AI/awesome-vision-language-navigation}{}
\DeclareTableWorkLinks{guo2024multiagentssurvey}{https://ijcai.org/proceedings/2024/890}{https://github.com/taichengguo/LLM_MultiAgents_Survey_Papers}{}
\DeclareTableWorkLinks{guo2026question}{https://arxiv.org/abs/2606.20683}{https://github.com/ggjy/Awesome-Agent-Engineering}{}
\DeclareTableWorkLinks{guo2026seeing}{https://arxiv.org/abs/2610.19366}{}{}
\DeclareTableWorkLinks{he2026workrover}{https://arxiv.org/abs/2610.18067}{}{}
\DeclareTableWorkLinks{hu2026raven}{https://arxiv.org/abs/2606.25206}{https://github.com/princeton-prism/RAVEN}{https://huggingface.co/datasets/zzcnewly/RAVEN_QA}
\DeclareTableWorkLinks{huang2026embodiedclbench}{https://arxiv.org/abs/2610.13021}{https://github.com/PKU-VaLuE-Lab/EmbodiedCLBench}{https://huggingface.co/datasets/PKU-VaLuE-Lab/EmbodiedCLBench}
\DeclareTableWorkLinks{ijcai2026p898}{https://ijcai.org/proceedings/2026/898}{}{}
\DeclareTableWorkLinks{jain2025words}{https://ijcai.org/proceedings/2025/1164}{}{}
\DeclareTableWorkLinks{jiang2026visualskill}{https://arxiv.org/abs/2606.18448}{https://github.com/XMHZZ2018/VisualSkills}{https://github.com/XMHZZ2018/VisualSkills/tree/main/skills}
\DeclareTableWorkLinks{johanns2026agentic}{https://arxiv.org/abs/2606.02080}{https://github.com/MMV-Lab/Agentic-J}{}
\DeclareTableWorkLinks{ju2026embodiskill}{https://arxiv.org/abs/2605.10332}{https://github.com/air-embodied-brain/EmbodiSkill}{https://github.com/air-embodied-brain/EmbodiSkill/tree/main/data/alfworld}
\DeclareTableWorkLinks{karten2026continual}{https://arxiv.org/abs/2605.09998}{https://github.com/sethkarten/continual-harness}{}
\DeclareTableWorkLinks{kong2026freeevolve}{https://arxiv.org/abs/2610.09197}{}{}
\DeclareTableWorkLinks{li2026comfyclaw}{https://arxiv.org/abs/2607.01709}{https://github.com/Moms-Organic-Agent-Lab/comfyclaw}{}
\DeclareTableWorkLinks{liu2026memory}{https://arxiv.org/abs/2606.31612}{}{}
\DeclareTableWorkLinks{liu2026osexpert}{https://arxiv.org/abs/2603.07978}{https://github.com/Lumos-Jiateng/OSExpert}{https://huggingface.co/datasets/Rushi2002/Expert}
\DeclareTableWorkLinks{liu2026path}{https://www.preprints.org/manuscript/202608.0051}{}{}
\DeclareTableWorkLinks{luo2026evogen}{https://arxiv.org/abs/2610.00383}{https://github.com/King-play/EvoGen-Harness}{}
\DeclareTableWorkLinks{ma2026tvir}{https://arxiv.org/abs/2606.02320}{https://github.com/NJU-LINK/TVIR}{}
\DeclareTableWorkLinks{meng2026agent}{https://www.preprints.org/manuscript/202604.0428/v3}{https://github.com/Gloriaameng/Awesome-Agent-Harness}{}
\DeclareTableWorkLinks{navasardyan2026failbench}{https://arxiv.org/abs/2609.03611}{}{}
\DeclareTableWorkLinks{ning2026codeharness}{https://arxiv.org/abs/2605.18747}{https://github.com/YennNing/Awesome-Code-as-Agent-Harness-Papers}{}
\DeclareTableWorkLinks{qiao2023reasoning}{https://aclanthology.org/2023.acl-long.294/}{https://github.com/zjunlp/Prompt4ReasoningPapers}{}
\DeclareTableWorkLinks{qin2024tool}{https://arxiv.org/abs/2304.08354}{https://github.com/OpenBMB/BMTools}{}
\DeclareTableWorkLinks{ren2026selfimprovements}{https://arxiv.org/abs/2607.13104}{https://github.com/selfimproving-agent/awesome-Self-Improving-Agents}{}
\DeclareTableWorkLinks{shirvani2026image}{https://arxiv.org/abs/2603.07455}{}{}
\DeclareTableWorkLinks{this-survey}{}{https://github.com/heshuting555/Awesome-Visual-Agent}{}
\DeclareTableWorkLinks{tian2026physevo}{https://arxiv.org/abs/2610.08995}{}{}
\DeclareTableWorkLinks{wang2023voyager}{https://arxiv.org/abs/2305.16291}{https://github.com/MineDojo/Voyager}{}
\DeclareTableWorkLinks{wei2026scale}{https://arxiv.org/abs/2609.39304v4}{}{}
\DeclareTableWorkLinks{xiao2026geoforge}{https://arxiv.org/abs/2608.10494}{}{}
\DeclareTableWorkLinks{xie2026mineevolve}{https://arxiv.org/abs/2603.13131}{https://github.com/xzw-ustc/MC-MineEvolve}{}
\DeclareTableWorkLinks{xing2026agenticvisualgeneration}{https://www.preprints.org/manuscript/202609.0173/v2}{}{}
\DeclareTableWorkLinks{xu2026evolvinggraphs}{https://arxiv.org/abs/2608.18104}{https://github.com/LuckyGirl-XU/Awesome-Agent-Dynamic-Graphs}{}
\DeclareTableWorkLinks{xu2026harness}{https://arxiv.org/abs/2610.14224}{https://github.com/google-research/harness2}{}
\DeclareTableWorkLinks{yu2026harness}{https://www.preprints.org/manuscript/202610.2293/v1}{}{}
\DeclareTableWorkLinks{zhang2024vlmvisionsurvey}{https://arxiv.org/abs/2304.00685}{https://github.com/jingyi0000/VLM_survey}{}
\DeclareTableWorkLinks{zhu2026hybrid}{https://arxiv.org/abs/2603.10291}{https://github.com/NickSiboZhu/HyMEM-GUI-Agent}{}
\DeclareTableWorkLinks{bousmalis2023robocat}{https://arxiv.org/abs/2306.11706}{}{}
\DeclareTableWorkLinks{added_mendonca2025continuously}{https://proceedings.mlr.press/v270/mendonca25a.html}{}{}




\DeclareTableWorkLinks{zhong2026actionengine}{https://arxiv.org/abs/2602.20502v1}{}{}

\DeclareTableWorkLinks{ICLR2026DeepEyes}{https://arxiv.org/abs/2505.14362v3}{}{}

\DeclareTableWorkLinks{ICLR2026Selfimprovingb}{https://arxiv.org/abs/2511.00091}{}{}

\DeclareTableWorkLinks{ICLR2026Wmpo}{https://arxiv.org/abs/2511.09515}{}{}

\DeclareTableWorkLinks{NeurIPS2026RePOVLA}{https://arxiv.org/abs/2605.09410}{}{}

\DeclareTableWorkLinks{NeurIPS2026ToolCUA}{https://arxiv.org/abs/2605.12481}{}{}

\DeclareTableWorkLinks{ICLR2026Simulation}{https://proceedings.iclr.cc/paper_files/paper/2026/hash/53b43ba4d5e12174a34ab94f9485df76-Abstract-Conference.html}{}{}

\DeclareTableWorkLinks{CVPR2026ProofofPerception}{https://arxiv.org/abs/2603.00324}{https://github.com/AryaFayyazi/PoP}{}

\DeclareTableWorkLinks{CVPR2026Recurrent}{https://arxiv.org/abs/2603.17312}{}{}

\DeclareTableWorkLinks{ICLR2026Webgenagent}{https://arxiv.org/abs/2509.22644}{}{}

\DeclareTableWorkLinks{CVPR2026Diagnose}{https://openaccess.thecvf.com/content/CVPR2026/html/Zeng_Diagnose_Correct_and_Learn_from_Manipulation_Failures_via_Visual_Symbols_CVPR_2026_paper.html}{}{}

\DeclareTableWorkLinks{CVPR2026MemoryAugmented}{https://openaccess.thecvf.com/content/CVPR2026/html/Zhou_Memory-Augmented_Scene_Understanding_and_Exploration_for_Open-World_Aerial_Object-Goal_Navigation_CVPR_2026_paper.html}{}{}

\DeclareTableWorkLinks{CVPR2026AstraNavMemory}{https://arxiv.org/abs/2512.21627}{}{}

\DeclareTableWorkLinks{ACL2026MMMem}{https://aclanthology.org/2026.acl-long.533/}{}{}

\DeclareTableWorkLinks{ACL2026MaDS}{https://aclanthology.org/2026.acl-long.1202/}{}{}

\DeclareTableWorkLinks{yang2026task}{https://arxiv.org/abs/2610.20100}{}{}

\DeclareTableWorkLinks{ACL2026VeriGUI}{https://aclanthology.org/2026.acl-long.1335/}{}{}

\DeclareTableWorkLinks{guo2026qreflectorlearningguiaction}{https://arxiv.org/abs/2608.05587}{}{}

\DeclareTableWorkLinks{sager2026comprehensive}{https://jair.org/index.php/jair/article/view/19490}{}{}

% Newly activated and added Visual Agent papers.
\DeclareTableWorkLinks{ACL2026GUI0}{https://aclanthology.org/2026.acl-long.2052/}{}{}
\DeclareTableWorkLinks{ICLR2026Genie}{https://arxiv.org/abs/2508.05635}{}{}
\DeclareTableWorkLinks{NeurIPS2026Autonomous}{https://arxiv.org/abs/2602.10356}{}{}
\DeclareTableWorkLinks{bai2026practice}{https://arxiv.org/abs/2608.30760}{https://github.com/BAAI-Agents/PRACTICE}{}
\DeclareTableWorkLinks{bundele2026trackers}{https://arxiv.org/abs/2610.15929}{}{}
\DeclareTableWorkLinks{che2026lvmh}{https://arxiv.org/abs/2610.23904}{}{}
\DeclareTableWorkLinks{che2026resight}{https://arxiv.org/abs/2610.33487}{}{}
\DeclareTableWorkLinks{deng2026training}{https://openaccess.thecvf.com/content/CVPR2026/html/Deng_Training_High-Level_Schedulers_with_Execution-Feedback_Reinforcement_Learning_for_Long-Horizon_GUI_CVPR_2026_paper.html}{}{}
\DeclareTableWorkLinks{jeong2026draft}{https://arxiv.org/abs/2511.11005}{https://github.com/EavnJeong/Draft-and-Refine-with-Visual-Experts}{}
\DeclareTableWorkLinks{jiang2026manimagent}{https://arxiv.org/abs/2606.30296v3}{}{}
\DeclareTableWorkLinks{kang2026simworld}{https://arxiv.org/abs/2605.09423v2}{}{}
\DeclareTableWorkLinks{karli2026recall}{https://arxiv.org/abs/2606.23617}{}{}
\DeclareTableWorkLinks{li2026magicgui}{https://arxiv.org/abs/2601.13060}{}{}
\DeclareTableWorkLinks{added_liu2026continualvla}{https://proceedings.mlr.press/v306/liu26bu.html}{}{}
\DeclareTableWorkLinks{liu2026rsigen}{https://arxiv.org/abs/2610.18688v2}{}{}
\DeclareTableWorkLinks{luo2026video}{https://arxiv.org/abs/2609.37950v1}{}{}
\DeclareTableWorkLinks{mishra2026tampagent}{https://arxiv.org/abs/2611.03584}{}{}
\DeclareTableWorkLinks{raghavan2026does}{https://arxiv.org/abs/2610.00542}{}{}
\DeclareTableWorkLinks{added_sun2026seagent}{https://proceedings.mlr.press/v306/sun26w.html}{}{}
\DeclareTableWorkLinks{tang2026trinity}{https://arxiv.org/abs/2610.36077v2}{https://github.com/InfRec-Cardinal/The-Trinity}{}
\DeclareTableWorkLinks{tian2026abot}{https://arxiv.org/abs/2607.10350v3}{}{}
\DeclareTableWorkLinks{wang2026atlasva}{https://arxiv.org/abs/2605.17933}{}{}
\DeclareTableWorkLinks{wang2026self}{https://arxiv.org/abs/2608.11350v2}{}{}
\DeclareTableWorkLinks{wang2026vevo}{https://arxiv.org/abs/2610.39158v1}{}{}
\DeclareTableWorkLinks{wei2026fate}{https://arxiv.org/abs/2603.01505}{}{}
\DeclareTableWorkLinks{xie2026preact}{https://arxiv.org/abs/2610.04916}{}{}
\DeclareTableWorkLinks{xie2026riwanav}{https://arxiv.org/abs/2610.08640}{}{}
\DeclareTableWorkLinks{xin2026agentvln}{https://arxiv.org/abs/2603.17670}{}{}
\DeclareTableWorkLinks{xu2026videoharness}{https://arxiv.org/abs/2608.24302v2}{}{}
\DeclareTableWorkLinks{ye2026videoresearcher}{https://arxiv.org/abs/2609.19664}{}{}
\DeclareTableWorkLinks{zeng2026visa}{https://arxiv.org/abs/2608.26013v2}{}{}
\DeclareTableWorkLinks{zhang2026pixelcraft}{https://arxiv.org/abs/2509.25185}{}{}
\DeclareTableWorkLinks{zhang2026rewardharness}{https://arxiv.org/abs/2605.08703}{https://github.com/TIGER-AI-Lab/RewardHarness}{https://huggingface.co/datasets/AgPerry/EditReward-Data-100}
\DeclareTableWorkLinks{zhou2026automating}{https://arxiv.org/abs/2606.30111v3}{}{}
\DeclareTableWorkLinks{zhu2026can}{https://arxiv.org/abs/2605.26820v3}{}{https://github.com/Agentic-Intelligence-Lab/RoboNever}
\DeclareTableWorkLinks{agashe2026evolving}{https://arxiv.org/abs/2610.28601}{}{}
\DeclareTableWorkLinks{chen2026kpharness}{https://arxiv.org/abs/2610.27417}{https://github.com/chenzk202212/adaptive-gaming-harnesses}{https://huggingface.co/datasets/cccsds/openha-minecraft-eval-149}
\DeclareTableWorkLinks{chen2026reflect}{https://arxiv.org/abs/2609.17653}{}{}
\DeclareTableWorkLinks{du2026designer}{https://arxiv.org/abs/2609.22086}{}{}
\DeclareTableWorkLinks{du2026from}{https://arxiv.org/abs/2610.29560}{}{}
\DeclareTableWorkLinks{fan2026skill}{https://arxiv.org/abs/2606.18890}{}{}
\DeclareTableWorkLinks{fang2026find}{https://arxiv.org/abs/2609.32069}{}{}
\DeclareTableWorkLinks{feng2026enactopt}{https://arxiv.org/abs/2610.14977}{}{}
\DeclareTableWorkLinks{ge2026make}{https://arxiv.org/abs/2609.39018}{}{}
\DeclareTableWorkLinks{hu2026interaction}{https://arxiv.org/abs/2609.04869}{}{}
\DeclareTableWorkLinks{huang2026work2skill}{https://arxiv.org/abs/2610.12984}{}{}
\DeclareTableWorkLinks{jiang2026grounded}{https://arxiv.org/abs/2610.13164}{}{}
\DeclareTableWorkLinks{lassoued2026orca}{https://arxiv.org/abs/2603.02438}{}{}
\DeclareTableWorkLinks{li2026knowact}{https://arxiv.org/abs/2607.12625}{}{}
\DeclareTableWorkLinks{li2026reflect}{https://arxiv.org/abs/2610.20312}{}{}
\DeclareTableWorkLinks{li2026sees}{https://arxiv.org/abs/2609.32698}{}{}
\DeclareTableWorkLinks{liu2026pilot}{https://arxiv.org/abs/2610.14335}{}{}
\DeclareTableWorkLinks{liu2026skilllens}{https://arxiv.org/abs/2608.10775}{}{}
\DeclareTableWorkLinks{luo2026instagent}{https://arxiv.org/abs/2610.23098}{}{}
\DeclareTableWorkLinks{refresh_scene2demo2026}{https://arxiv.org/abs/2602.12065v3}{}{}
\DeclareTableWorkLinks{song2026embodiedrsi}{https://arxiv.org/abs/2610.10498}{}{}
\DeclareTableWorkLinks{tharwat2026dream}{https://arxiv.org/abs/2610.13816}{}{}
\DeclareTableWorkLinks{wang2026visualevolve}{https://arxiv.org/abs/2610.28386}{}{}
\DeclareTableWorkLinks{wen2026forkcast}{https://arxiv.org/abs/2610.18650}{}{}
\DeclareTableWorkLinks{xu2026artisancad}{https://arxiv.org/abs/2607.05750}{}{}
\DeclareTableWorkLinks{xu2026videoevoharness}{https://arxiv.org/abs/2610.15389}{https://github.com/Wei-Xin-Xu/VideoEvoHarness}{}
\DeclareTableWorkLinks{yang2026gui}{https://arxiv.org/abs/2610.00948}{}{}
\DeclareTableWorkLinks{yang2026self}{https://arxiv.org/abs/2610.15084}{https://github.com/YWenxi/marvo}{}
\DeclareTableWorkLinks{zhang2026cineevolve}{https://arxiv.org/abs/2610.29590}{}{}
\DeclareTableWorkLinks{zhang2026imagining}{https://arxiv.org/abs/2608.14822}{}{}
\DeclareTableWorkLinks{zhao2026echopath}{https://arxiv.org/abs/2609.16635}{}{}
\DeclareTableWorkLinks{zhao2026making}{https://arxiv.org/abs/2604.15917}{}{}

% Newly activated and added Visual Agent papers.
\DeclareTableWorkLinks{AAAI2026Connecting}{https://arxiv.org/abs/2511.19516}{}{}
\DeclareTableWorkLinks{AAAI2026CorrectAD}{https://arxiv.org/html/2511.13297}{}{}
\DeclareTableWorkLinks{AAAI2026DigimonGPT}{https://ojs.aaai.org/index.php/AAAI/article/view/37523}{}{}
\DeclareTableWorkLinks{AAAI2026Guieyes}{https://ojs.aaai.org/index.php/AAAI/article/view/40175}{}{}
\DeclareTableWorkLinks{AAAI2026HistoryAware}{https://ojs.aaai.org/index.php/AAAI/article/view/40966}{}{}
\DeclareTableWorkLinks{AAAI2026Rethinking}{https://ojs.aaai.org/index.php/AAAI/article/view/37337}{}{}
\DeclareTableWorkLinks{AAAI2026Seqwalker}{https://arxiv.org/html/2601.04699}{}{}
\DeclareTableWorkLinks{AAAI2026TCoT}{https://ojs.aaai.org/index.php/AAAI/article/view/37577}{https://github.com/Serenos/TCoT}{}
\DeclareTableWorkLinks{AAAI2026Talk2Image}{https://ojs.aaai.org/index.php/AAAI/article/view/40519}{}{}
\DeclareTableWorkLinks{AAAI2026Worldagen}{https://ojs.aaai.org/index.php/AAAI/article/download/38925/42887}{}{}
\DeclareTableWorkLinks{ACL2026Breaking}{https://arxiv.org/html/2508.07642v4}{}{}
\DeclareTableWorkLinks{ACL2026DocVStar}{https://aclanthology.org/2026.acl-long.2129/}{}{}
\DeclareTableWorkLinks{ACL2026LookLess}{https://arxiv.org/abs/2510.01681}{}{}
\DeclareTableWorkLinks{ACL2026MAGNET}{https://arxiv.org/abs/2601.19199}{}{}
\DeclareTableWorkLinks{ACL2026ModelBasedImagination}{https://aclanthology.org/2026.acl-long.827.pdf}{}{}
\DeclareTableWorkLinks{ACL2026OSSentinel}{https://aclanthology.org/2026.acl-long.431/}{}{}
\DeclareTableWorkLinks{ACL2026RSMeM}{https://arxiv.org/html/2607.24772}{}{}
\DeclareTableWorkLinks{ACL2026SimpleVGC}{https://aclanthology.org/volumes/2026.acl-long/}{}{}
\DeclareTableWorkLinks{ACL2026UICopilot}{https://aclanthology.org/2026.acl-long.904/}{}{}
\DeclareTableWorkLinks{CVPR2026ActiveVLA}{https://arxiv.org/abs/2601.08325}{}{}
\DeclareTableWorkLinks{CVPR2026AgentDet}{https://openaccess.thecvf.com/content/CVPR2026/html/Li_AgentDet_A_Shared-Blackboard_Multi-Agent_Framework_for_Zero-Few-Shot_Object_Detection_CVPR_2026_paper.html}{}{}
\DeclareTableWorkLinks{CVPR2026AtomicVLA}{https://openaccess.thecvf.com/content/CVPR2026/supplemental/Zhang_AtomicVLA_Unlocking_the_CVPR_2026_supplemental.pdf}{}{}
\DeclareTableWorkLinks{CVPR2026CGL}{https://arxiv.org/abs/2603.02951}{}{}
\DeclareTableWorkLinks{CVPR2026CodeDance}{https://arxiv.org/abs/2512.17312}{}{}
\DeclareTableWorkLinks{CVPR2026Counterfactual}{https://arxiv.org/abs/2512.24426}{}{}
\DeclareTableWorkLinks{CVPR2026DRSGUI}{https://arxiv.org/abs/2605.15542}{}{}
\DeclareTableWorkLinks{CVPR2026Experience}{https://arxiv.org/html/2604.05533}{}{}
\DeclareTableWorkLinks{CVPR2026ForeAct}{https://arxiv.org/abs/2602.12322}{}{}
\DeclareTableWorkLinks{CVPR2026GUISAGE}{https://openaccess.thecvf.com/content/CVPR2026/papers/Tang_GUI-SAGE_Enhancing_GUI_Automation_with_Self-Explanatory_Learning_CVPR_2026_paper.pdf}{}{}
\DeclareTableWorkLinks{CVPR2026HATS}{https://arxiv.org/abs/2603.12138}{}{}
\DeclareTableWorkLinks{CVPR2026Learning}{https://arxiv.org/html/2605.31365}{}{}
\DeclareTableWorkLinks{CVPR2026Learningto}{https://arxiv.org/html/2505.20289}{}{}
\DeclareTableWorkLinks{CVPR2026LensWalk}{https://arxiv.org/abs/2603.24558}{}{}
\DeclareTableWorkLinks{CVPR2026OctoT2I}{https://arxiv.org/abs/2606.01803}{}{}
\DeclareTableWorkLinks{CVPR2026REACH}{https://openaccess.thecvf.com/content/CVPR2026/html/Ke_REACH_Explicit_Recovery_Behavior_for_Diffusion_Policies_CVPR_2026_paper.html}{}{}
\DeclareTableWorkLinks{CVPR2026RoboAgent}{https://openaccess.thecvf.com/content/CVPR2026/html/Xu_RoboAgent_Chaining_Basic_Capabilities_for_Embodied_Task_Planning_CVPR_2026_paper.html}{}{}
\DeclareTableWorkLinks{CVPR2026SaPaVe}{https://arxiv.org/abs/2603.12193}{}{}
\DeclareTableWorkLinks{ICLR2026Adareasoner}{https://proceedings.iclr.cc/paper_files/paper/2026/hash/e6f8759254d86ea9c197d30b92b313ca-Abstract-Conference.html}{}{}
\DeclareTableWorkLinks{ICLR2026Earthagent}{https://arxiv.org/abs/2509.23141}{}{}
\DeclareTableWorkLinks{ICLR2026Embodied}{https://openreview.net/pdf?id=E5L43l5EIu}{}{}
\DeclareTableWorkLinks{ICLR2026FilMaster}{https://arxiv.org/abs/2506.18899}{}{}
\DeclareTableWorkLinks{ICLR2026Generative}{https://openreview.net/pdf?id=DM0Y0oL33T}{}{}
\DeclareTableWorkLinks{ICLR2026Lets}{https://proceedings.iclr.cc/paper_files/paper/2026/hash/3e1fb72d876d634b2ac29e9ac2c937c9-Abstract-Conference.html}{}{}
\DeclareTableWorkLinks{ICLR2026MATA}{https://arxiv.org/abs/2601.19204}{}{}
\DeclareTableWorkLinks{ICLR2026Planning}{https://openreview.net/pdf/6082975fa8793aee0005fc28ab58c5ebfcd2eb8c.pdf}{}{}
\DeclareTableWorkLinks{ICLR2026Pursuing}{https://arxiv.org/abs/2510.16688}{}{}
\DeclareTableWorkLinks{ICLR2026RWoM}{https://arxiv.org/html/2510.11892}{}{}
\DeclareTableWorkLinks{ICLR2026Selfimprovinga}{https://proceedings.iclr.cc/paper_files/paper/2026/hash/cde874a797a8300da693d5e412b7fdc0-Abstract-Conference.html}{}{}
\DeclareTableWorkLinks{ICLR2026Sparse}{https://arxiv.org/abs/2506.01392}{}{}
\DeclareTableWorkLinks{ICLR2026Transductive}{https://transductive-visualprogram.github.io/}{}{}
\DeclareTableWorkLinks{ICLR2026Videozoomer}{https://arxiv.org/abs/2512.22315}{}{}
\DeclareTableWorkLinks{ICML2026Agent0VL}{https://arxiv.org/abs/2511.19900}{https://github.com/aiming-lab/Agent0}{}
\DeclareTableWorkLinks{ICML2026CoEvolving}{https://proceedings.mlr.press/v306/wang26kz.html}{}{}
\DeclareTableWorkLinks{ICML2026Reason}{https://proceedings.mlr.press/v306/wang26hh.html}{}{}
\DeclareTableWorkLinks{ICML2026VABS}{https://arxiv.org/abs/2605.10172}{}{}
\DeclareTableWorkLinks{NeurIPS2026APIVOT}{https://arxiv.org/html/2607.08024}{}{}
\DeclareTableWorkLinks{NeurIPS2026AdaptiveImagine}{https://arxiv.org/abs/2602.08236}{}{}
\DeclareTableWorkLinks{NeurIPS2026ECHO}{https://arxiv.org/html/2605.10993}{}{}
\DeclareTableWorkLinks{NeurIPS2026GenEvolve}{https://arxiv.org/abs/2605.21605}{}{}
\DeclareTableWorkLinks{NeurIPS2026MMSkills}{https://arxiv.org/abs/2605.13527}{}{}
\DeclareTableWorkLinks{NeurIPS2026VLAPro}{https://arxiv.org/abs/2605.29562}{}{}
\DeclareTableWorkLinks{NeurIPS2026VideoTrees}{https://arxiv.org/abs/2607.16189}{}{}
\DeclareTableWorkLinks{added_kim2026race}{https://proceedings.iclr.cc/paper_files/paper/2026/hash/fab80bb9d97e9b9ff5c19f91f72838c6-Abstract-Conference.html}{}{}
\DeclareTableWorkLinks{added_li2026deepscan}{https://arxiv.org/abs/2603.03857}{}{}
\DeclareTableWorkLinks{added_wang2026highfrequency}{https://arxiv.org/html/2605.24931}{}{}
\DeclareTableWorkLinks{added_wang2026remac}{https://arxiv.org/abs/2601.20130}{}{}
\DeclareTableWorkLinks{added_yu2026mact}{https://openaccess.thecvf.com/content/CVPR2026/html/Yu_Visual_Document_Understanding_and_Reasoning_A_Multi-Agent_Collaboration_Framework_with_CVPR_2026_paper.html}{}{}

% Newly activated and added Visual Agent papers.
\DeclareTableWorkLinks{CVPR2026A}{https://arxiv.org/abs/2603.14052}{https://github.com/git-disl/A4VL}{}

% Remaining Table III papers; URLs retained from references_added.bib.
% Recursive-update table additions: paper links are the cited public records;
% code links are included only where an official public repository was identified.
\DeclareTableWorkLinks{wang2026adarsi}{https://arxiv.org/abs/2610.20474}{}{}
\DeclareTableWorkLinks{wang2026regenharness}{https://arxiv.org/abs/2609.27612}{}{}
\DeclareTableWorkLinks{wang2026harnesspai}{https://arxiv.org/abs/2609.29166}{https://github.com/Darwin-Agent/HarnessPAI}{}
\DeclareTableWorkLinks{gao2026recurir}{https://arxiv.org/abs/2611.18006}{}{}
\DeclareTableWorkLinks{jiang2026harnessmmv}{https://xsci.com/preprint/doi/10.66977/xsci.2611.000p}{https://github.com/YuhuaJiang2002/HarnessMM}{}
\DeclareTableWorkLinks{jiang2026wovr}{https://arxiv.org/abs/2602.13977v3}{https://github.com/RLinf/RLinf}{}
\DeclareTableWorkLinks{yu2026coda}{https://arxiv.org/abs/2610.22362}{}{}
\DeclareTableWorkLinks{lee2026revision3d}{https://arxiv.org/abs/2609.32984v2}{}{}
\DeclareTableWorkLinks{jiang2026skillrubric}{https://arxiv.org/abs/2609.34557}{}{}
\DeclareTableWorkLinks{jian2026learning}{https://arxiv.org/abs/2610.41865}{}{}
\DeclareTableWorkLinks{wang2026vericua}{https://arxiv.org/abs/2610.26469}{https://github.com/Jeffjeno/VeriCUA}{}
\DeclareTableWorkLinks{tan2026getting}{https://arxiv.org/abs/2610.14852}{}{}
\DeclareTableWorkLinks{sui2026learning}{https://arxiv.org/abs/2605.16857v2}{https://github.com/XingYuSSS/AutoMMemo}{}
\DeclareTableWorkLinks{baermann2026forget}{https://arxiv.org/abs/2604.11306v2}{}{}
\DeclareTableWorkLinks{xu2026videoevolve}{https://arxiv.org/abs/2610.10183}{}{}
\DeclareTableWorkLinks{zou2026taskmem}{https://arxiv.org/abs/2605.31075}{https://github.com/ByteDance-Seed/TaskMem}{}
\DeclareTableWorkLinks{zhang2026flex}{https://arxiv.org/abs/2611.08946v1}{https://github.com/flex-rsi/rsi-bench}{https://huggingface.co/datasets/Flex-RSI/RSI-Dataset}
\DeclareTableWorkLinks{li2026physical}{https://arxiv.org/abs/2610.26848v1}{https://github.com/PhysRSI-Eval/PhysRSI-Eval-code}{}
\DeclareTableWorkLinks{chi2026ai4ai}{https://arxiv.org/abs/2608.20318v1}{https://github.com/Einsia/AI4AI-Bench}{}
\DeclareTableWorkLinks{rsi-exam-2026}{https://rsi-exam.ai/}{https://github.com/aiming-lab/RSI-Exam}{https://huggingface.co/datasets/RSI-Exam/RSI-Exam}
\DeclareTableWorkLinks{openrsi2026index}{https://index.openrsi.foundation/}{https://github.com/OpenRSI-Foundation/OpenRSI-Index}{https://huggingface.co/datasets/OpenRSI-Foundation/OpenRSI-Index-Logs}
\DeclareTableWorkLinks{ramesh2026autoresearchexam}{https://benchmarks.bespokelabs.ai/autoresearchexam/}{https://github.com/bespokelabsai/AutoResearchExam}{}
\DeclareTableWorkLinks{valsai2026rsiindex}{https://vals-ai.com/benchmarks/rsi_index}{}{}

